Deterministic Variational Inference for Robust Bayesian Neural Networks

Bayesian neural networks (BNNs) hold great promise as a flexible and principled solution to deal with uncertainty when learning from finite data. Among approaches to realize probabilistic inference in deep neural networks, variational Bayes (VB) is theoretically grounded, generally applicable, and computationally efficient. With wide recognition of potential advantages, why is it that variational Bayes has seen very limited practical use for BNNs in real applications? We argue that variational inference in neural networks is fragile: successful implementations require careful initialization and tuning of prior variances, as well as controlling the variance of Monte Carlo gradient estimates. We provide two innovations that aim to turn VB into a robust inference tool for Bayesian neural networks: first, we introduce a novel deterministic method to approximate moments in neural networks, eliminating gradient variance; second, we introduce a hierarchical prior for parameters and a novel Empirical Bayes procedure for automatically selecting prior variances. Combining these two innovations, the resulting method is highly efficient and robust. On the application of heteroscedastic regression we demonstrate good predictive performance over alternative approaches.

==> content/section_old_dvi.tex <==
\section{Deterministic Approximation of a Bayesian Neural Network}
\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{resources/architecture.pdf}
	\caption{\todo{}}
	\label{fig:architecture}
\end{figure}
\Figref{fig:architecture} shows the architecture of the computation of $\E_{\weights \sim q}\left[\log p(\data|\weights)\right]$ for a feed forward neural network. The computation can be divided into two parts, namely propagation of activations though parametrized layers (blue) and evaluation of an unparametrized log-likelihood function ($\likelihood$). In the following sections, we describe how each of these stages is handled in our deterministic framework.

\subsection{Moment Propagation}
\label{sec:propagation}
\begin{wrapfigure}{R}{0.4\textwidth}
	\centering
	\includegraphics[width=0.38\textwidth]{resources/approximation.pdf}
	\caption{\todo{}}
	\label{fig:approximation}
\end{wrapfigure}
We begin by considering activation propagation illustrated in \figref{fig:architecture}(a), with the aim of deriving the form of the distribution $\hidden^L$ that will be passed to the likelihood computation. We compute $\hidden^L$ by sequentially computing the distributions for the activations in the preceding layers. Concretely, we define the action of the $\ell^{\rm th}$ layer that maps $\hidden^{(\ell-1)}$ to $\hidden^\ell$ as follows:
\begin{align}
\activation^{\ell} &= f(\hidden^{(\ell-1)}) \nonumber\\
\hidden^\ell &= \activation^\ell\layerweights^\ell+\layerbias^\ell,
\label{eqn:layer}
\end{align}
where $f$ is a nonlinearity and $\{\layerweights^\ell, \layerbias^\ell\}\subset \weights$ are random variables representing the weights and biases of the $\ell^{\rm th}$ layer that are assumed independent of weights in other layers. For notational clarity, in the following we will suppress the explicit layer index $\ell$ and use primed symbols to denote variables from the $(\ell-1)^{\rm th}$ layer. Note that the definition in \eqref{eqn:layer} is subtley distinct from the traditional definintion\footnote{Setting the nonlinearity of the $0^{\rm th}$ layer to the identity as shown in \figref{fig:architecture} and re-drawing the boundaries of the layers recovers a traditional architecture where the nonlinearity \emph{follows} the linear transformation.}
 $\smash{\hidden=f\left(\hidden' \layerweights^\ell + \layerbias^\ell\right)}$, to highlight that $\hidden$ is a linear combination of the elements of the nonlinearly transformed activations $\activation$. In the limit of vanishing correlation between terms in this combination, we appeal to the central limit theorem (CLT) to argue that the sum of random variables $\smash{\sum_j a_j W_{ji}}$ in the computation of $\smash{\hidden_i}$ will be normally distributed for large hidden dimensions regardless of the potentially complicated disribution for $\smash{a_j}$ induced by $f$. Then, choosing a Gaussian variational approximation for $\layerbias$ leaves $\hidden$ also Gaussian, and we empirically observe that this claim is approximately valid even when (weak) correlations appear between the elements of $\activation$ during training.

Having argued the Gaussian form for $\hidden$, it remains to compute its first and second moments. In general, these cannot be computed exactly, so we develop an approximate expression. An overview of this derivation is presented here with more details in the appendix. First, we model $\layerweights$, $\layerbias$ and $\activation$ as independent random variables, allowing us to write:
\begin{align}
\expectation{h_i} &= \expectation{a_j}\expectation{W_{ji}} + \expectation{b_i} \nonumber\\
\Cov(h_i, h_k) &= \expectation{a_j a_l}\Cov(W_{ji},W_{lk}) 
                         + \expectation{W_{ji}}\Cov(a_j, a_l)\expectation{W_{lk}}
                         + \Cov(b_i, b_k),
\label{eqn:propagation}
\end{align}
where we have employed the Einstein summation convention and used angle brackets to indicate expectation over $q$. If we choose a variational family with analytic forms for weight means and covariances (e.g. Gaussian), then the only difficult terms are the moments of $\activation$:
\begin{align}
\expectation{a_j} &\propto \int f(h) \exp\left[
	-\tfrac{h-\expectation{h'_j}}{2\Sigma'_{jj}}
\right] \; \fulld h\
\label{eqn:firstmoment}
\\
\expectation{a_j a_l} &\propto \int f(g)f(h) \exp\left[-
	\frac{1}{2}
	\begin{psmallmatrix}g - \expectation{h'_j} \\h - \expectation{h'_l}\end{psmallmatrix}^T
	\begin{psmallmatrix}\Sigma'_{jj} & \Sigma'_{jl} \\ \Sigma'_{lj} & \Sigma'_{ll}\end{psmallmatrix}^{-1}
	\begin{psmallmatrix}g - \expectation{h'_j} \\h - \expectation{h'_l}\end{psmallmatrix}
\right] \;\fulld g\fulld h,
\label{eqn:secondmoment}
\end{align}
where we have used the Gaussian form of $\hidden'$ parameterized by mean $\expectation{\hidden'}$ and covariance $\bm{\Sigma'}$, and for brevity we have omitted the normalizing constants. For Heaviside or ReLU choices of nonlinearity $f$ closed form solutions for the integral in \eqref{eqn:firstmoment} exists in terms of error functions. Furthermore, for these nonlinearities, the $\expectation{\hidden'_j}\to \pm\infty$ and $\expectation{\hidden'_l}\to \pm\infty$ asymptotes of the integral in \eqref{eqn:secondmoment} have analytical form. \Figref{fig:approximation} shows how these asympotes can be used as a first approximation for \eqref{eqn:secondmoment}. This approximation is improved by considering that by definition, the residual decays to zero far from the origin in the $(\expectation{\hidden'_j}, \expectation{\hidden'_l})$ plane, and so is well modelled by a decaying function $\smash{\exp[-Q(\expectation{\hidden'_j}, \expectation{\hidden'_l}, {\bm \Sigma'})]}$, where $Q$ is a polynomial in $\smash{\expectation{\hidden'_{j,l}}}$ with a dominant positive even term. In practice we truncate $Q$ at the quadratic term, and calculate the polynomial coefficients by matching the moments of the resulting Gaussian with the analytical moments of the residual (see \todo{supplementary}). Specifically, when we adopt dimensionless variables $\smash{\mu'_i = \expectation{\hidden'_i} / \sqrt{\Sigma'_{ii}}}$ and $\smash{\rho'_{ij} = \Sigma'_{ij}/\sqrt{\Sigma'_{ii}\Sigma'_{jj}}}$, this improved approximation takes the form
%
\begin{align}
\expectation{a_j a_l} &= \frac{\Sigma'_{jl}}{\rho'_{jl}}\left\{A(\mu_j', \mu_l', \rho_{jl}') + \exp\left[-Q(\mu_j', \mu_l', \rho_{jl}')\right]\right\},
\label{eqn:theapproximation}
\end{align}
where the expressions for the asymptote $A$ and quadratic $Q$ are given in table \tabref{tab:approximation} and derived in the \todo{supplementary}.
\begin{table}
\centering
\begin{tabular}{M{0.4in}M{1.1in}M{3.5in}}
\toprule
			& 
	$A(\mu_1, \mu_2, \rho)$   &
	$Q(\mu_1, \mu_2, \rho)$ \\
\midrule
Heaviside	& 
	$\Phi(\mu_1)\Phi(\mu_2)$ & 
	$-\log(\frac{g_h}{2\pi})+\frac{\rho}{2g_h\bar{\rho}}\left[\mu_1^2+\mu_2^2-\frac{2\rho}{1+\bar{\rho}}\mu_1\mu_2\right] +\mathcal{O}(\mu^4)$ \\
ReLU		& 
	$\softrelu(\mu_1)\softrelu(\mu_2)$\newline \phantom{.}\hspace{0.3cm}$+\;\rho\Phi(\mu_1)\Phi(\mu_2)$ & 
	$-\log(\frac{g_r}{2\pi}) + \left[\frac{\rho}{2g_r(1+\bar{\rho})}\left(\mu_1^2+\mu_2^2\right)-\frac{\sin^{-1}(\rho)-\rho}{g_r\rho}\mu_1\mu_2\right]+\mathcal{O}(\mu^4)$\\
\bottomrule
\end{tabular}
\caption{Forms for the components of the approximation in \eqref{eqn:theapproximation} for Heaviside and ReLU nonlinearities. $\Phi$ is the CDF of a standard Gaussian, SR is a ``soft ReLU'' that we define as $\softrelu(x)=\phi(x)+x\Phi(x)$ where $\phi$ is a standard Gaussian, $\smash{\bar{\rho} = \sqrt{1-\rho^2}}$, $\smash{g_h = \sin^{-1}(\rho)}$ and $\smash{g_r = g_h + \frac{\rho}{1+\bar{\rho}}}$  }
\label{tab:approximation}
\end{table}

Using \eqref{eqn:theapproximation} in \eqref{eqn:propagation} gives a closed form approximation for the moments of $\hidden$ given moments of $\hidden'$. Since $\hidden$ is approximately normally distributed by the CLT, this is sufficient information to sequentially propagate moments all the way through the network to compute $\hidden^L$. Any deep learning framework with gradients implemented for $\sin^{-1}$ and $\Phi$ will immediately support backpropagation through the deterministic expressions we have presented. Below we briefly empirically verify this approximate form and in \secref{??} we will show how it is used to compute a log-likelihood for training.

\subsubsection{Empirical Verification of Approximation}
\begin{wrapfigure}{r}{0.5\textwidth}
	\centering
	\includegraphics[width=0.48\textwidth]{resources/toy_data.pdf}
	\caption{\todo{}}
	\label{fig:toy}
\end{wrapfigure}
The approximation derived above relies on two assumptions \todo{also assume independence of layers}. First, that some form of CLT theorem holds for the hidden units during training where the iid assumption of the classic CLT is not strictly enforced. Second, that a quadratic truncation of $Q$ is sufficient\footnote{Additional Taylor expansion terms can be computed if this assumtion fails.}. To provide evidence that these assumptions hold in practice, we train a small ReLU network with two hidden layers each of 128 units to perform 1D heteroskedastic regression on a toy dataset of 500 points drawn from the distribution shown in \figref{fig:toy}(b). Details of the training procedure follow those in \secref{sec:??}, and here it is sufficient to note that $\hidden^L$ in this network is a 2-element vector where the elements are labelled as $(m, \ell)$. We use a diagonal gaussian variational family to represent the weights, but we preserve the full covariance of $\hidden$ during propagation. Using an input $x=0.25$ we compute the distributions for $m$ and $\ell$ both at the start of training (where we expect the iid assumption to hold) and at convergence (where iid does not necessarily hold). \Figref{fig:toy}(c) shows the comparison between $\hidden^L$ distributions reported by our deterministic approximation and MC evaluation using 20k samples from $\vardist$. This comparison is qualitatively excellent for all cases considered.

\subsection{Log-likelihood Evaluation}
To use the moment propagation procedure derived above for training BNNs, we need to build a function $\likelihood$ that maps from $\hidden^L$ to the reconstruction term of the ELBO in \eqref{eqn:elbo}: i.e. the expected log-likelihood of the observed data (see \figref{fig:architecture}(b)). We begin by rewriting the reconstruction term in the ELBO as follows for a data point $(\rvx, y)$:
\begin{align}
	\E_{\weights\sim q}\left[\log p(y|\weights)\right] 
	= \int \log p(y|\weights) q(\weights) \;\fulld\weights 
	= \int \log p(y|\weights) p(\weights|\hidden^L) p(\hidden^L) \;\fulld\weights \fulld\hidden^L,
\end{align}
where we have suppressed explicit conditioning on $\rvx$ for brevity. Our goal now is to perform the integral over $\weights$ to write the expectation in terms of $\hidden^L$ only, thus allowing it to be evaluated using the approximation to $p(\hidden^L)$ from the previous section.

To eliminate $\weights$, consider the case where the output of the model is a distribution $p(y|\hidden^L)$ that is a parameter-free transformation of $\hidden^L$ (e.g. $\hidden^L$ are logits of a softmax distribution for classification or the moments of a Gaussian for regression). Since the model output is conditioned only on $\hidden^L$, we must have $p(y|\weights) = p(y|\hidden^L)$ for all configurations $\weights$ that satisfy the deterministic transformation $\hidden^L=\model(\rvx;\weights)$, where $\model$ is the neural network (i.e $p(y|\weights) = p(y|\hidden^L)$ for all $\weights$ where $p(\weights|\hidden^L)$ is non-zero). This allows us to write:
\begin{align}
	\int \log p(y|\rvx, \weights) p(\weights|\hidden^L) \;\fulld\weights = \log p(y|\hidden^L)\int p(\weights|\hidden^L) \;\fulld\weights = \log p(y|\hidden^L),
\end{align}
so the reconstruction term becomes:
\begin{align}
	\E_{\weights\sim q}\left[\log p(y|\rvx, \weights)\right] 
	= \int \log p(y|\hidden^L) p(\hidden^L) \fulld\hidden^L
	= \E_{\hidden^L\sim p(\hidden^L)}\left[\log p(y|\hidden^L)\right].
\label{eqn:variableExchange}
\end{align}

\todo{}

\subsubsection{Regression}
For simplicity we consider scalar\footnote{\todo{see supplementary for higher dimensional regression}} $y$ and a Gaussian noise model parameterized by mean $m(\rvx)$ and heteroscedastic log-variance $[\log\sigma^2_y(\rvx)]=\ell(\rvx)$. The parameters of this Gaussian are read off as the elements of a 2-dimensional output layer $\hidden^L=(m,\ell)$ - i.e. $p(y|\hidden^L) = \normal\left[y|m, e^\ell\right]$. Recall that these parameters themselves are uncertain and the statistics $\expectation{\hidden^L}$ and $\bfSigma^L$ can be computed following \secref{sec:propagation}. Inserting the Gaussian forms for $p(y|\hidden^L)$ and $p(\hidden^L)$ into \eqref{eqn:variableExchange} and performing the integral (see \todo{supplementary}) gives a closed form expression for the ELBO reconstruction term:
\begin{align}
	\E_{\hidden^L\sim p(\hidden^L)}\left[\log p(y|\hidden^L)\right] 
	= -\tfrac{1}{2}\left[
		\log 2\pi 
		+ \expectation{l} 
		+ \tfrac{\Sigma_{mm}+\left(\expectation{m}-\Sigma_{m\ell}-y\right)^2}
				{e^{\expectation{l}-\Sigma_{\ell\ell}/2}}\right].
\label{eqn:regLikelihood}
\end{align}
This heteroscedastic model can be made homoscedastic by setting $\Sigma_{\ell\ell} = \Sigma_{m\ell} = 0$. The expression in \eqref{eqn:regLikelihood} completes the derivations required to implement the closed form approximation to the ELBO reconstruction term for training a network. In addition, we can also compute a closed form for the predictive distribution (see \todo{supplementary}) that can be used at test-time to produce predictions that encorporate all parameter uncertainties.
\begin{align}
	p(y) = \int p(y|\hidden^L)p(\hidden^L) \;d\hidden^L = \normal\left(y|m, \Sigma_{mm}+e^{\expectation{l}+\Sigma_{\ell\ell}/2}\right)
\end{align}


%\section{Application of Moment Computation to Variational Bayes}\label{app}
%In this section, we apply the approximate Gaussian distribution by using the moment computation technique (sec.~\ref{mc}) to variational Bayes. 
%\subsection{Regression}
%Denote the Gaussian distribution of the last hidden activation $\rvh$ as $r(\rvh)\sim\mathcal{N}(\rvh|\bm{\mu}_\rvh,\bfSigma_{\rvh})$. For Gaussian observational noise, we have $\rvy\sim\mathcal{N}(\rvy|\rvh,\sigma^2)$ where $\sigma^2$ is the noise variance. The expectation term in eq.~\ref{elbo} turns into $\mathbb{E}_{r(\rvh)}[\mbox{log} \mathcal{N}(\rvy|\rvh,\sigma^2)]$ which has an analytical expression,
%\begin{eqnarray}
%\mathbb{E}_{r(\rvh)}[\mbox{log} \mathcal{N}(\rvy|\rvh,\sigma^2)]=-\frac{(\bm{\mu}_\rvh-\rvy)^\top(\bm{\mu}_\rvh-\rvy)}{2\sigma^2}-\frac{1}{2\sigma^2}\mbox{Tr}(\bfSigma_\rvh)-\frac{d}{2}\log2\pi\sigma^2
%\end{eqnarray}
%where $d$ is the number of hidden units in $\rvh$.
%
%Similarly, the marginal distribution of $\rvy$ is
%\begin{eqnarray}
%p(\rvy)=\int p(\rvy|\rvx,\rvw)p(\rvw)d\rvw\approx\int p(\rvy|\rvh)r(\rvh)d\rvh=\mathcal{N}(\rvy|\bm{\mu}_{\rvh},\bfSigma_{\rvh}+\sigma^2\rmI_d)
%\end{eqnarray}
%The posterior distribution of $\rvw$ is
%\begin{eqnarray}
%p(\rvw|\rvx,\rvy)\approx q_{\bm{\theta}^*}(\rvw)=\mathcal{N}(\rvw|\bm{\mu}^*,{\bfSigma^*}^2)
%\end{eqnarray}
%where $\bm{\theta}=\{\bm{\mu},\bfSigma^2\}$.
%
%Given a new input vector $\rvx_{\star}$, the prediction of its output $\rvy_{\star}$ is
%\begin{eqnarray}
%p(\rvy_{\star}|\rvx_{\star},\rvx,\rvy)=\int p(\rvy_{\star}|\rvx_{\star},\rvw)p(\rvw|\rvx,\rvy)d\rvw\approx\int p(\rvy_{\star}|\rvh_{\star})r(\rvh_{\star})d\rvh_{\star}=\mathcal{N}(\rvy_{\star}|\bm{\mu}_{\rvh_{\star}},\bfSigma_{\rvh_{\star}}+\sigma^2\rmI_d)
%\end{eqnarray}
%where $r(\rvh_{\star})=\mathcal{N}(\rvh_{\star}|\bm{\mu}_{\rvh_{\star}},\bfSigma_{\rvh_{\star}})$ is derived using the deterministic approximation given the Gaussian distribution $p(\rvw|\rvx,\rvy)$ for $\rvw$. Therefore we are also able to obtain a closed-form posterior predictive distribution for a new input.
%
%\subsubsection{Heteroscedastic Model}
%Considering Gaussian noise for regression, we can easily extend homoscedastic model with singular $\sigma^2$ to heteroscedastic model with data dependent noise. Let $\rvy\sim\mathcal{N}(\rvh,\mbox{exp}(\rvl))$, where $\rvl$ is another hidden activation from the neural net. The joint Gaussian distribution of $\rvh$ and $\rvl$ can be written as
%\begin{eqnarray}
%\left[\begin{matrix}
%\rvh\\
%\rvl
%\end{matrix}\right]\sim\mathcal{N}\bigg(\left[\begin{matrix}
%\bm{\mu}_\rvh\\
%\bm{\mu}_\rvl
%\end{matrix}\right], \left[\begin{matrix}
%\bfSigma_{\rvh\rvh}&\bfSigma_{\rvh\rvl}\\
%\bfSigma_{\rvh\rvl}^\top&\bfSigma_{\rvl\rvl}
%\end{matrix}\right]\bigg).
%\end{eqnarray}
%
%The expectation term in eq.~\ref{elbo} still maintains a closed-form expression,
%\begin{eqnarray}
%&&\mathbb{E}_{r(\rvh,\rvl)}[\mbox{log}\mathcal{N}(\rvy|\rvh,\mbox{exp}(\rvl))]=-\frac{d}{2}\log2\pi-\frac{1}{2}\sum_i(\bm{\mu}_\rvl)_i\\
%&&-\frac{1}{2}\sum_i\mbox{exp}\left(-(\bm{\mu}_\rvl)_i+\frac{1}{2}(\bfSigma_{\rvl\rvl})_{ii}\right)\bigg[(\bfSigma_{\rvh\rvh})_{ii}+\Big((\bm{\mu}_\rvh-\rvy)_i-(\bfSigma_{\rvh\rvl})_{ii}\Big)^2\bigg]
%\end{eqnarray}
%
%Correspondingly, the posterior predictive becomes
%\begin{eqnarray}
%p(\rvy_{\star}|\rvx_{\star},\rvx,\rvy)\approx\int p(\rvy_{\star}|\rvh_{\star},\rvl_{\star})r(\rvh_{\star},\rvl_{\star})d\rvh_{\star}d\rvl_{\star}
%\end{eqnarray}
%which can be approximated by a one-layer Monte Carlo integration. 

\subsubsection{Classification}
Experiments in this paper focus on regression where no approximation is required in the computation of the reconstruction term and the predictive distribution. For softmax classification with logits $\hidden^L$ we do not find exact forms, however, using the delta method (see \todo{supplementary}) we find expansions
\begin{align*}
	\E_{\hidden^L\sim p(\hidden^L)}\left[\log p(y|\hidden^L)\right]
	&= \expectation{\hidden^L} - \E_{\hidden^L\sim p(\hidden^L)}\left[\logsumexp(\hidden^L)\right]\\
	&\approx \expectation{\hidden^L} - \logsumexp(\expectation{\hidden^L}) + \tfrac{1}{2}\left(\mathbf{p}^{\rm T} \diag(\bfSigma^L) - \mathbf{p}^{\rm T} \bfSigma^L\mathbf{p}\right), \\[1em]
	p(y) = \E_{\hidden^L\sim p(\hidden^L)}\left[p(y|\hidden^L)\right] &\approx \mathbf{p}\odot\left[1 + \mathbf{p}^{\rm T} \bfSigma^L\mathbf{p} - \bfSigma^L\mathbf{p} + \tfrac{1}{2}\diag(\bfSigma^L) - \tfrac{1}{2}\mathbf{p}\odot\diag(\bfSigma^L)\right].
\end{align*}
where $\mathbf{p} = {\rm softmax}(\hidden^L)$. Preliminary experiments show that good results are obtained either using these approximations or a lightweight MC approximation just to perform the mapping of $\hidden^L$ to $(\log)\mathbf{p}$ after the heavyweight work of computing $\hidden^L$ is done deterministically. In this work we are primarily concerned with demonstrating the benefits of the moment propagation method from \secref{sec:propagation}, so we limit our experiments to regression examples without additional complication from approximation of the likelihood function.


%
%\subsection{Classification}
%Although we focus on regression in this paper, we can relax the closed form with one-layer Monte Carlo integration in order to generalize to more output distributions, e.g. softmax classification. The idea is propagating Gaussian distributions all the way to the last hidden layer before the output.
%\begin{eqnarray}
%\mathbb{E}_{q(\rvw)}[\mbox{log} p(\rvy|\rvx,\rvw)]\approx\mathbb{E}_{r(\rvh)}[\mbox{log}p(\rvy|\rvh)]\approx\sum_{l=1}^L \mbox{log}p(\rvy|\rvh^l), \quad \rvh^l \sim r(\rvh)
%\end{eqnarray}
%For Gaussian regression, it enables other nonlinear functions than exponential function for heteroscedastic variance. It also allows more general distributions and more tasks using Bayesian neural networks.

==> content/section_old_empirical_bayes.tex <==
\section{Empirical Bayes for Variational BNNs}
\label{sec:eb}
So far, we have described methods for deterministic approximation of the reconstruction term in the ELBO. We now turn to the KL term. For a $d$-dimensional Gaussian prior $p(\weights)=\normal[\bm{\mu}_{\rm p}, \bfSigma_{\rm p}]$, the KL divergence with the Gaussian variational distribution $q=\normal[\bm{\mu}_{\rm q}, \bfSigma_{\rm q}]$ has closed form:
\begin{equation}
	\KLdiv{q}{p} = \tfrac{1}{2}\left[
		\log\tfrac{|\bfSigma_{\rm p}|}{|\bfSigma_{\rm q}|}
		- d
		+ \Tr\left(\bfSigma_{\rm p}^{-1}\bfSigma_{\rm q}\right)
		+ (\bm{\mu}_{\rm p} - \bm{\mu}_{\rm q})^{\rm T}\bfSigma_{\rm p}^{-1}(\bm{\mu}_{\rm p} - \bm{\mu}_{\rm q})
	\right].
	\label{eqn:KLterm}
\end{equation}
However, this requires selection of $(\mu_{\rm p}, \bfSigma_{\rm p})$ for which there is usually little intuition beyond arguing $\bm{\mu}_{\rm p} = \bm{0}$ by symmetry and choosing $\bfSigma_{\rm p}$ to preserve the expected magnitude of the propagating activations \citep{Xavier, He}.
%
In practice, variational Bayes for neural network parameters is quite sensitive to the choice of variance parameters, and we will demonstrate this problem empirically in Section \todo{Add section reference}.

To make variational Bayes robust we propose to parametrize the prior hierarchically, retaining a conditional diagonal Gaussian prior and variational distribution on the weights.  The hierarchical prior takes the form $\rvs \sim p(\rvs); \weights \sim p(\weights | \rvs)$, using an inverse gamma distribution on $\rvs$ as the conjugate prior to the elements of the diagonal Gaussian variance. We partition the weights into sets that typically coincide with the layer partitioning\footnote{In general, any arbitrary partitioning can be used}, and assign a single element in $\rvs$ to each set:
\begin{align}
	s_\lambda &\sim \invgamma(\alpha,\beta), \quad(\mbox{shape } \alpha \mbox{ and scale } \beta)\nonumber\\
	w^\lambda_i &\sim \normal(0, s_\lambda)
	\label{eqn:ebdist}
\end{align}
where $w^\lambda_i$ is the $i^{\rm th}$ weight in set $\lambda$.

Rather than taking the fully Bayesian approach of forming the prior by marginalization: $p(w_i^\lambda) = \int p(w_i^\lambda|s^\lambda)p(s^\lambda)\;\fulld s^\lambda$, we adopt an \emph{empirical} Bayes approach assuming that this integral is dominated by a contribution from an optimal value $s^\lambda=s^\lambda_*$. We use the data to inform the optimal setting of $s^\lambda_*$ to produce the tightest ELBO \todo{add some more intuition here?}:
\begin{align}
	&{\rm ELBO} = \E_{\weights\sim q}\left[\log p(y|\hidden^L)\right] - \left\{\KLdiv{q}{p(\weights|\rvs_*)p(\rvs_*)}\right\}\nonumber\\
	&\qquad \implies s^\lambda_* = \argmin_{s^\lambda}\left\{\KLdiv{q}{p(\weights^\lambda|s^\lambda)p(s^\lambda)}\right\}
	\label{eqn:ebelbo}
\end{align}
Writing out the integral for the KL in \eqref{eqn:ebelbo}, substituting in the forms of the distributions in \eqref{eqn:ebdist} and differentiating to find the optimum gives
\begin{align}
s^\lambda_*=\tfrac{\Tr\left[\bfSigma^\lambda_{\rm q} + \bm{\mu}^\lambda_{\rm q}(\bm{\mu}_{\rm q}^\lambda)^{\rm T}\right]+2\beta}{W^\lambda+2\alpha+2},
\end{align}
where $W^\lambda$ is the number of weights in the set $\lambda$. The influence of the data on the choice of $s^\lambda_*$ is made explicit here through dependence on the variational parameters $\bfSigma_{\rm q}$ and $\bm{\mu}_{\rm q}$. Using $s^\lambda_*$ to populate the elements of the diagonal prior variance $\bfSigma_{\rm p}$, we can evaluate the KL in \eqref{eqn:KLterm} under the empirical Bayes prior. Optimization of the resulting ELBO then simultaneously tunes the variational distribution and prior, and in practice we find minimal manual tuning of the hyperprior parameters $\alpha$ and $\beta$ are required \todo{say something about the rough values that work?}.
